Eider: Empowering Document-level Relation Extraction with Efficient Evidence Extraction and Inference-stage Fusion

Document-level relation extraction (DocRE) aims to extract semantic relations among entity pairs in a document. Typical DocRE methods blindly take the full document as input, while a subset of the sentences in the document, noted as the evidence, are often sufficient for humans to predict the relation of an entity pair. In this paper, we propose an evidence-enhanced framework, Eider, that empowers DocRE by efficiently extracting evidence and effectively fusing the extracted evidence in inference. We first jointly train an RE model with a lightweight evidence extraction model, which is efficient in both memory and runtime. Empirically, even training the evidence model on silver labels constructed by our heuristic rules can lead to better RE performance. We further design a simple yet effective inference process that makes RE predictions on both extracted evidence and the full document, then fuses the predictions through a blending layer. This allows Eider to focus on important sentences while still having access to the complete information in the document. Extensive experiments show that Eider outperforms state-of-the-art methods on three benchmark datasets (e.g., by 1.37/1.26 Ign F1/F1 on DocRED).

==> introduction_1112.tex <==
\section{Introduction}
Relation extraction~(RE) is the task of extracting semantic relations among entities within a given text, which has abundant applications such as knowledge graph construction, question answering, and biomedical text analysis \citep{yu-etal-2017-improved,Shi2019DiscoveringHI,trisedya-etal-2019-neural}. 
Prior studies mostly focus on predicting the relation between entities in a single sentence.
However, in the reality, it is common that a relation can only be inferred given multiple sentences as the context.
As a result, recent studies have been moving towards the more realistic setting of document-level relation extraction (DocRE) \citep{quirk-poon-17-distant,peng-etal-17-cross,DBLP:conf/aaai/GuptaRSR19}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_intro.pdf}
    \upv
    \vspace{-0.5cm}
    \caption{ A test sample in the DocRED dataset \cite{DocRED-paper}, where the $i^{th}$ sentence in the document is marked with [i] at the start. Our model correctly predicts [1,10] as evidence, and if we only use the extracted evidence as input, the model can predict the relation ``country of origin'' correctly. }
    \label{fig_intro}
    \downv
\end{figure}


Contrary to typical DocRE models which blindly take the whole document as input, a human may only need a few sentences to infer the relation between two specific entities.
We define the minimal set of sentences required by human annotators to infer the relation of an entity pair as \textit{evidence sentences} \cite{DocRED-paper}.
As shown in Figure~\ref{fig_intro}, to predict the relation between \textit{``Hero of the Day''} and \textit{``the United States''}, it is sufficient to know \textit{Load (the album)} was released in \textit{the United States} from the $1^{st}$ sentence, and \textit{``Hero of the Day''} is a single of \textit{Load} from the $10^{th}$ sentence. In other words, the $1^{st}$ and $10^{th}$ sentences serve as evidence sentences of this entity pair.
Although the $9^{th}$ sentence also mentions \textit{``the United States''}, it is irrelevant to this specific relation. Including such irrelevant sentences in input might sometimes introduce noise to the model and be more detrimental than beneficial.

In light of the observations above, 
we propose an \textbf{e}v\textbf{id}ence-\textbf{e}nhanced \textbf{R}E framework \ours, which makes better use of evidence in both training and inference.
For training, we improve DocRE by jointly extracting relations and evidence using multi-task learning.
Namely, the two tasks have their own classifier and share the base encoder.
Intuitively, both tasks should focus on the information relevant to the current entity pair, such as the underlined \textit{``Load''} and \textit{``the album''} in the $1^{st}$ and $10^{th}$ sentence of Figure~\ref{fig_intro}. 
This suggests that the two tasks have certain commonalities and can provide additional training signals for each other.

One may raise the concern that training an additional task could result in massive training time and memory overhead. For instance, \citet{E2GRE} requires around 10 times as long as training the RE task alone and cannot be trained on a single consumer GPU.
Furthermore, relying heavily on evidence annotation, as \citet{E2GRE}, may also limit the method's generalizability.
To reduce training time and memory, we use the same sentence representation for all relations and only train the evidence extraction model on entity pairs with at least one relation.
Empirically, our joint model requires only around 5\% additional training time and 14\% more memory compared to the individual RE model.
In case human annotation of evidence is not accessible, we design several heuristic rules to construct silver labels.
Experiments show that our method still improves RE performance even trained with silver labels.


With the evidence extracted in training, we
further enhance DocRE by focusing more on the extracted evidence in inference.
In the extreme case, if there is only one sentence related to the relation prediction, we can make predictions solely based on this sentence and reduce the problem to sentence-level relation extraction.
One concurrent study \cite{3Sent} raises the possibility of replacing the full document with a few sentences extracted by rules.
However, their method does not achieve consistent improvements. 
Since the rules cannot perfectly recover the evidence, solely relying on the extracted sentences may miss important information and harm model performance in certain cases (see Table~\ref{tab:ablation}).
Instead, we construct a pseudo document by concatenating all the extracted evidence sentences and make RE predictions on both the pseudo and original documents. Then we fuse the two predictions using a blending layer \citep{Blending}. In this way, \ours puts more attention to the extracted important sentences, while still having access to the whole document to avoid information loss.




We conduct extensive experiments on three widely-adopted DocRE benchmarks: DocRED \cite{DocRED-paper}, CDR \cite{CDR} and GDA \cite{GDA}.
Experiment results show that \ours achieves state-of-the-art performance on all the datasets.
Performance analysis further shows that the improvement of \ours is most significant on inter-sentence entity pairs, suggesting that leveraging evidence is especially effective in reasoning over multiple sentences.
In particular, \ours significantly improves the performance on entity pairs that require co-reference/multi-hop reasoning by 1.98/2.08 F1 on DocRED, respectively.


\start{Contributions}
(1) We propose an efficient joint relation and evidence extraction model that allows the two tasks to mutually enhance each other with negligible computational overhead, which does not heavily rely on evidence annotation
(2) We design a simple and effective evidence-enhanced inference method for DocRE, which allows the model to focus more on the important sentences with no information loss
(3) We demonstrate that our evidence-enhanced framework outperforms state-of-the-art methods on three DocRE datasets.


==> introduction_orig.tex <==
\section{Introduction}
Relation extraction~(RE) is the task of extracting semantic relations among entities within a given text, which has abundant applications such as knowledge graph construction, question answering, and biomedical text analysis~\citep{yu-etal-2017-improved,Shi2019DiscoveringHI,trisedya-etal-2019-neural}. 
Prior studies mostly focus on predicting the relation between entities in a single sentence.
However, in the reality, it is common that a relation can only be inferred given multiple sentences as the context.
As a result, recent studies have been moving towards the more realistic setting of document-level relation extraction~(DocRE) \citep{quirk-poon-17-distant,peng-etal-17-cross,DBLP:conf/aaai/GuptaRSR19}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_intro.pdf}
    \upv
    \vspace{-0.5cm}
    \caption{ A test sample in the DocRED dataset \cite{DocRED-paper}, where the $i^{th}$ sentence in the document is marked with [i] at the start. Our model correctly predicts [1,4] as evidence, and if we only use the extracted evidence as input, the model can predict the relation ``Country'' and ``Located in'' correctly. }
    \label{fig_intro}
    \downv
\end{figure}


In each document, the sentences are not \textit{equally important} for each entity pair and some sentences could be irrelevant for the relation prediction. 
For each entity pair, we refer to the minimal set of sentences required to infer their relation as \textit{evidence sentences} \cite{DocRED-paper}.
As shown in Figure~\ref{fig_intro}, to predict the relation between \textit{``Ontario''} and \textit{``Canada''}, it is sufficient to know \textit{Paul Desmarais} is a \textit{Canadian} from the $1^{st}$ sentence, and \textit{Paul Desmarais} was born in \textit{Ontario} from the $4^{th}$ one. In other words, the $1^{st}$ and $4^{th}$ sentences serve as evidence sentences of this entity pair.
Although the $2^{nd}$ and $3^{rd}$ sentences lie between these two sentences, they are irrelevant to this specific relation. Including such irrelevant sentences in input might sometimes introduce noise to the model and be more detrimental than beneficial.

In light of the observations above, we propose two approaches to make better use of evidence sentences. The first is to combine evidence in inference.
One naive way is to directly make predictions on the evidence sentences, as in~\cite{3Sent}. 
However, other sentences may also include relevant information, such as the information of the involved entities.
Discarding all other sentences may result in loss of coherence and harm model performance in certain cases.
Hence, we fuse the prediction results of the original document and evidence to highlighting the most important sentences while avoiding information loss. Notice that this method does not need additional training and can be applied to general DocRE models.

In case evidence sentences are not provided in inference, they can be extracted by training an evidence extracted model using multi-task learning.
This also serves as our second approach to improve DocRE with evidence.
Intuitively, both tasks should focus on the information relevant to the current entity pair, such as the underlined \textit{``Paul Desmarais''} and \textit{``Desmarais''} in the $4^{th}$ sentence of Figure~\ref{fig_intro}. 
This suggests that the two tasks have certain commonalities and can provide additional training signals for each other.
To avoid the massive training time and memory overhead due to training an additional task, our model adopts a simpler model structure and is trained on only part of the evidence annotation, which requires only ~5\% additional training time and ~14\% more memory. 
When human-annotated evidence sentences are not available even for training, we find that a simple set of heuristic rules can serve to construct silver labels with relatively high quality.
Experiment results show that even the model trained with silver labels can outperform the baseline significantly.

In this paper, we propose an \textbf{e}v\textbf{id}ence-\textbf{e}nhanced \textbf{R}E framework \ours, which automatically extracts evidence and effectively leverages the extracted evidence to improve the performance of DocRE.
We first train a relation extraction model and an evidence extraction model using multi-task learning. If the human-annotated evidence is not accessible even in training, we adopt several heuristic rules to construct silver labels instead.
To reduce memory usage and training time, we use the same sentence representation across relations and only train the evidence extraction model on positive entity pairs with at least one relation.
During inference, we construct a pseudo document by concatenating all the evidence (or predicted evidence). Finally, we fuse the predictions based on the original document and the pseudo document using a blending layer~\citep{Blending}. 






Extensive experiments show that \ours outperforms the state-of-the-art methods on widely-adopted DocRE benchmarks DocRED~\cite{DocRED-paper}, CDR~\cite{CDR} and GDA~\cite{GDA}.
Further examination shows that the improvement of \ours is especially large on inter-sentence entity pairs, 
where multiple sentences are involved.

\start{Contributions}
(1) We propose an evidence-empowered inference process of DocRE, which improves the performance without re-training the RE model.
(2) We jointly learn relation and evidence extraction using multi-task learning, where the two tasks mutually enhance each other.
(3) In the absence of human-annotated evidence labels, we design a set of rules to construct evidence labels and show that these silver labels can already improve DocRE performance.
(4) We demonstrate that \ours outperforms state-of-the-art methods on three DocRE datasets: DocRED, CDR, and GDA.
